Krylov Subspace Recycling For Matrix Functions

We derive an augmented Krylov subspace method with subspace recycling for computing a sequence of matrix function applications on a set of vectors. The matrix is either fixed or changes as the sequence progresses. We assume consecutive matrices are closely related, but make no assumptions on the relationship between the vectors. We present three versions of the method with different practical implementations. We demonstrate the effectiveness of the method using a range of numerical experiments with a selection of functions and matrices. We primarily focus our attention on the sign function arising in the overlap formalism of lattice QCD.

==> old_experiments.tex <==
\section{Numerical experiments}\label{numericalexperiments}
In this section we present results of our numerical experiments. These experiments aim to test the effectiveness of all three implementations of r(FOM)$^{2}$ as both an augmented Krylov subspace method, and as a method for recycling. Our experiments require knowledge of an exact solution for a sequence of slowly changing matrices, and have thus been limited to relatively small problem sizes. 

We compare the results of r(FOM)$^{2}$ to the standard Arnoldi approximation (\ref{Arnoldi_Cauchy:eq}). For the evaluation of the matrix function on the small $j \times j$ and $(j+k) \times (j+k)$ matrices in standard Arnoldi and version~3 (line \ref{line:mat_eval} in \Cref{version3:alg}), respectively, we use a ``direct'' method, given by an appropriate built-in Matlab function.  These MATLAB functions also allow us to obtain what we considered the ``exact'' solution for each experiment which we used to determine the error. 
Our experiments, in addition, compute the Arnoldi approximation evaluated using the same quadrature procedure on the Hessenberg matrix as r(FOM)$^{2}$ (denoted Arnoldi (q)).

All experiments involving the sign function have been performed using a $4^{4}$ lattice QCD matrix $D$ of size $3072 \times 3072$ taken from 
the SuiteSparse Matrix Collection \cite{Davis2011} (matrix ID 1591). Since practical QCD computations represent the sign function in terms of the inverse square root function, our experiments report results on evaluation of the inverse square root function instead.

%In some experiments we work with the Hermitian matrix $ Q = \Gamma_{5} D$, and since the sign function is typically computed using the relation $\sign(Q) = (Q^2)^{-1/2} Q$, our experiments actually report the results for the inverse square root of $Q^2$, which can be represented as a Stieltjes integral (see \Cref{sec:stieltjes})
%\[
%z^{-1/2} = \frac{-1}{\pi} \int_{-\infty}^{0} \frac{\sigma^{-1/2}}{\sigma-z} d \sigma,
%\]
%for which we use a variant of Gaussian quadrature as detailed in \cite{frommer2014efficient}.
 
 
For all other functions tested we take the contour of integration $\Gamma$ to be a circle of radius $r$ centered at the point $c$ and use the trapezoidal rule for numerical integration. The contour $\Gamma$ is given by the parameterization
\[
     %\{ \Gamma = z \in \mathbb{C} \hspace{0.1cm}| \hspace{0.1cm} 
     z = r e^{i \theta} + c, \hspace{0.3cm} 0 \leq \theta \leq 2 \pi 
     %\}
     ,
\]
and the nodes of the trapezoidal rule are the 
$n_\quadp$ equidistant points 
given by
\[
    z_{\ell} = r e^{i \theta_{\ell}} + c \hspace{0.1cm}, \hspace{0.1cm} \theta_{\ell} = \ell \Delta \theta, \hspace{0.1cm} \ell = 0,1,.., n_{quad} - 1, \enspace \Delta \theta = 2 \pi/n_{quad}.
\]
Since $\Gamma$ is closed, the trapezoidal rule is particularly accurate and features exponential convergence; see \cite{Trefethen14,Weideman02}, e.g.

\subsection{Results}

\begin{figure}
   \centering
    \subfloat[\centering]
    {{\includegraphics[width=6cm]{sign_augmentation_result.png} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=6cm]{inverseLQCDm40k20.png} }}%
    \qquad 
     \subfloat[\centering]{{\includegraphics[width=6cm]{logchemicalpotential10000x10000m40k20.png} }}%
      \qquad 
      \subfloat[\centering]{{\includegraphics[width=6cm]{sqrtpoissonm40k20.png} }}%
      \qquad 
     \caption{
     Comparison of Arnoldi and the three versions of r(FOM)$^{2}$ for computing $f(A)\vb.$ QCD examples: (a) $f(z) = z^{-\frac{1}{2}}$ and $A = Q^{2}$, (b) $f(z) = \frac{1}{z}$  and $A = D$. Finite difference examples: (c)  $f(z) = \mbox{log}(z)$ and $A$ a 2d convection diffusion matrix %of size $10,000 \times 10,000$, 
     (d) $f(z) = \sqrt{z}$ and $A$ discrete Laplace matrix. % of size $10,000 x 10,000$. 
     All experiments use $j=40$ Arnoldi iterations and recycle space dimension $k = 20$.}%
     \label{fig:augmentation_test}%
\end{figure}


\Cref{fig:augmentation_test} shows the results obtained from augmenting the Krylov subspace with high quality eigenvector approximations computed directly from the matrix $A$. We compared the three versions of r(FOM)$^{2}$ (denoted $\widetilde{f}_{1}, \widetilde{f}_{2}$ and $\widetilde{f}_{3}$ respectively) to the the standard Arnoldi approximation with ``direct'' evaluation of $f$ on the Hessenberg matrix (Arnoldi) and 
the quadrature based approximation (Arnoldi (q)). The experiments were run for a range of values for $n_{quad}$.

The experiment in \Cref{fig:augmentation_test} (a) corresponds to the inverse square root of $Q^{2}$. In \Cref{fig:augmentation_test} (b) we tested the method on the inverse function of the standard Wilson Dirac matrix $D$. Both these experiments show that all implementations of r(FOM)$^{2}$ lead to a significant reduction in the error as compared to the Arnoldi approximation. The experiments in \Cref{fig:augmentation_test} (c/d) further demonstrate the effectiveness of r(FOM)$^{2}$ using rather academic examples for which the standard Arnoldi approximation performs poorly, while r(FOM)$^{2}$ significantly increases the quality of the approximation. In (c) we compute the log function of a matrix arising from a second order finite difference discretization of a 2D convection diffusion problem on a $100 \times 100$ mesh, taken from the open source \textit{funm$\_$quad} code \cite{frommer2014efficient}. In (d) we compute the square root of the discrete Laplace matrix corresponding to a discretization of Poisson's equation on the unit square as given in the MATLAB test matrix gallery.


There are some common observations we can make from these experiments. Firstly, we observe that beyond a certain number of quadrature points, the error of quadrature Arnoldi stagnates and becomes identical to the error of standard Arnoldi. This indicates that the quadrature error has become negligible as compared to the subspace approximation error. For the augmented methods, one typically needs more quadrature points before such a stagnation occurs. 

At stagnation and beyond, the r(FOM)$^{2}$ approximations  significantly outperform the standard Arnoldi approximation and all three implementations produce the same approximation. We also note that the $\widetilde{f}_{3}$ approximation is more accurate than the other two versions
of r(FOM)$^{2}$ for the same number of quadrature points. 
This is because this approximation involves a term which does not depend on quadrature but a ``closed form'' evaluation of the function. The other two approximations are based entirely on quadrature and thus require a larger number of quadrature points to achieve the same level of accuracy. Even though time measurements cannot be regarded as conclusive with our implementations and software, we just mention that versions $2$ and $3$ tend to take somewhat longer compute time than version $1$, an 
observation which is in line with our cost analysis.



In \Cref{fig:example_via_inverse}, \ref{fig:sign_recycle} and \ref{fig:eigenvalues_quality} we demonstrate the effectiveness of the three versions of r(FOM)$^{2}$ as a recycle method. For each experiment we use enough quadrature points so that all three implementations produce the same approximation. We denote the common error curve for all implementations as r(FOM)$^{2}$ in the plots.


\begin{figure}
    \centering
    \subfloat[\centering  ]{{\includegraphics[width=6cm]{LQCDinveps0m50k20quad1000_common_approx.png} }}%
    \qquad
     \subfloat[\centering  ]{{\includegraphics[width=6cm]{LQCDinveps0001m50k20quad1000_common_approx.png} }}%
    \qquad 
     \caption{Comparison of standard Arnoldi and the three versions of r(FOM)$^{2}$ when applying the inverse of the $4^{4}$ lattice QCD matrix $D$ on a sequence of 10 random vectors. All experiments used $j=50$ Arnoldi iterations, a recycle subspace dimension $k = 20$ and $1000$ quadrature points. $\epsilon = 0$ in (a), $\epsilon = 10^{-3}$ in (b).}
    \label{fig:example_via_inverse}%
\end{figure}

The experiments in \Cref{fig:example_via_inverse} involve computing the inverse function on a sequence of slowly changing Wilson Dirac matrices against 10 random vectors.
We used a parameter $\epsilon$ to describe the strength of the perturbation between each matrix in the sequence. In  \Cref{fig:example_via_inverse} (a) we demonstrate the  result for  $\epsilon = 0$ which corresponds to the special case where the matrix $A^{(i)}$ remains fixed for all $i$, and only the vectors $\vb^{(i)}$ change throughout the sequence.
In \Cref{fig:example_via_inverse} (b) we demonstrate the case where the matrices now change according to a random perturbation of strength $\epsilon = 10^{-3}$. For all our experiments we make no assumption on the relationship between consecutive vectors $\vb^{(i)}$ and generate an independent random vector for each new problem in the sequence. The subspace $\mathcal{U}$ has been computed between each system using the harmonic Ritz procedure outlined in \Cref{harmritz}. In the plots below, enough quadrature points have been chosen so that the standard Arnoldi and the quadrature based Arnoldi produce the same approximation, and are thus represented as the same curve. From these experiments we see that all three variants of r(FOM)$^{2}$ exhibit significant reductions in error as compared to the standard Arnoldi approximation without recycling, and that they consistently reduce the error further as we move throughout the sequence of problems. This is one of the key qualities of an effective recycling method as outlined in \cite{parks2006recycling}.

\begin{figure}
    \centering
    \subfloat[\centering  ]{{\includegraphics[width=6cm]{eps0LQCD.png} }}%
    \qquad
     \subfloat[\centering  ]{{\includegraphics[width=6cm]{eps00001LQCD.png} }}%
    \qquad 
    \subfloat[\centering  ]{{\includegraphics[width=6cm]{eps0001LQCD.png} }}%
    \qquad 
     \subfloat[\centering  ]{{\includegraphics[width=6cm]{eps001LQCD.png} }}%
     \caption{Comparison of Arnoldi approximation with the 3 versions of r(FOM)$^{2}$ for a sequence of 30 applications of the inverse square root function with randomly changing matrices. The strength of change is controlled by $\epsilon$. 
     Fig (a) is for $\epsilon = 0$ (matrices remain constant), and $\epsilon = 10^{-4}$ in (b), $\epsilon = 10^{-3}$ in (c), and $\epsilon = 10^{-2}$ in (d). All experiments use $j=50$ Arnoldi iterations, recycle subspace dimension of size $k=20$ and $n_\quadp = 30$. 
     }
    \label{fig:sign_recycle}%
\end{figure}

 In \Cref{fig:sign_recycle} we repeat a similar experiment as in \Cref{fig:example_via_inverse}, but this time with 30 computations of $f(A^{(i)})\vb^{(i)}$ with $f$ the inverse square root, $A^{(1)} = Q^{2}$ and then producing a sequence of perturbed Hermitian matrices $A^{(i)}$ with the strength of change controlled by $\epsilon$ as in the previous experiment.  \Cref{fig:sign_recycle} (a/b/c) were performed with $\epsilon = 0$, $10^{-4}$ and $10^{-3}$, respectively, and demonstrate the same behaviour as observed in the previous experiment. The error is reduced considerably as we move along the sequence of matrix function applications.

\begin{figure}
    \centering
    \includegraphics[width=6cm]{eigs_test.png}
    \caption{Minimum eigenvalue for each $A^{(i)}$ in the experiments in \Cref{fig:sign_recycle} for the different values of $\epsilon$. For $\epsilon = 0.01$, negative eigenvalues appear from the $14^{th}$ system on.}
    \label{fig:eigenvalues_quality}
\end{figure}


 
The plot in \Cref{fig:sign_recycle} (d) has $\epsilon = 10^{-2}$. 
This experiment performs similarly to the other experiments up until problem index 14, where the random perturbations have caused the spectrum to shift to the negative real part of the complex plane (see \Cref{fig:eigenvalues_quality}). This highlights an important practical limitation of r(FOM)${}^2$: The contour of integration (which we consider to be the interval $(-\infty,0]$ in the Stieltjes case) needs to enclose the spectrum of the matrix. If this is not the case anymore, as in problem number 14, where $A$ has a negative eigenvalue, we do not compute the correct integral unless we adapt the contour $\Gamma$.  
This issue will be highly application dependent. It will  not pose an issue for applications where sets containing the spectra of all matrices involved are known in advance or for the special case where the matrix remains fixed.

We conclude with a larger-scale test, using a sequence of 20 matrices. This matrix sequence are consecutive in Monte Carlo time, taken
from a Hybrid Monte Carlo computation. They correspond to a $16^4$ lattice.  These systems each have 786,432 unknowns.  This test also approximates the matrix square root for each system in the sequence.  Due to the size of these systems, we cannot compute the true matrix square roots in order to calculate the error.  Instead, we estimate error by measuring the residual for the matrix square root.  In \Cref{fig:large_scale}, we see that r(FOM)$^{2}$ does exhibit a performance improvement over the Arnoldi method.  However, we observe that the residual convergence does stagnate, and this stagnation persist for the sequence of 20 problems.  This behavior persisted for a number of different realizations of this experiment with different recycled subspace sizes and different Krylov subspace dimensions.  We also experimented with real-scalar-shifting the matrices to move the spectrum closer and further from the imaginary axis, but this only effected performance when the shifts were unrealistically large and positive.  One hypothesis explaining this performance is that for these problems of this size, the implementation presented here suffers from some numerical issues.  

\begin{figure}
    \centering
    \includegraphics[width=7cm]{m50k25sig0.2.png}
    \caption{Results for a sequence of large-scale QCD problems. 
    }
    \label{fig:large_scale}
\end{figure}





\begin{figure}
    \centering
    \includegraphics[width=7cm]{U_test.png}
    \caption{Accuracy of the recycle subspace $\mathcal{U}$ as an eigenvector approximation from the experiments in \Cref{fig:sign_recycle}. 
    }
    \label{fig:quality_U}
\end{figure}


Finally, we demonstrate  how the recycle subspace $\mathcal{U}$ converges to a good approximate eigenspace for each of the problems in the sequence. This is one of the requirements for an effective recycled method outlined in \cite{parks2006recycling}. We demonstrate this in \Cref{fig:quality_U} using the recycle subspace $\mathcal{U}$
for each of the experiments in \Cref{fig:sign_recycle}. \Cref{fig:quality_U} shows how accurately the subspace $\mathcal{U}$ approximates the eigenvectors of $A$ as the sequence of matrix function applications progresses. This was measured by computing the angle $\theta (\mathcal{U},\mathcal{Z})$ between the subspace $\mathcal{U}$ and the subspace $\mathcal{Z}$  spanned by the $k$ smallest exact eigenvectors of each matrix $A^{(i)}$ in the sequence. 
In general, we see that the quality of the computed recycled subspace improves, i.e.\ $\theta (\mathcal{U},\mathcal{Z})$ becomes smaller, as the sequence progresses provided the matrices in the sequence are slowly changing. For a large enough perturbation of the matrix, the quality of $\mathcal{U}$ appears to remain roughly fixed throughout the sequence. 


\section{Conclusions}\label{conclusions}
In this paper we have presented a new algorithm  r(FOM)$^{2}$ for computing an augmented Krylov subspace approximation to the action of a matrix function on a vector; we have extended the technique of subspace recycling (allowing for augmentation and recycling of arbitrary subspace information) to the application of functions of sparse matrices. To our knowledge, this is the first such paper to offer a proof the viability of this concept.  The approximation allows one to recycle information between sequences of matrix function applications wherein the matrix and/or right hand side is changing. We presented three different implementation approaches and have demonstrated their effectiveness using numerical experiments. Our experiments suggest the method works very well as a recycling method, but has potential limitations when sufficient \textit{a priori} information of each matrix in the sequence is 
not available
This is not a major issue for most applications of interest such as Lattice QCD where we know where the spectrum is contained.
Our experiments show that the algorithms are effective and that this approach can work for treating approximating sequences of matrix function applications.  However, we have demonstrated that there are some limitations for larger-scale, ill-conditioned matrices, and further investigation is necessary to obtain the same sort of convergence behavior as for the smaller-scale problems. 



==> replies.tex <==
\noindent{\Large Replies to referees}

\medskip

We would like to thank the referee for their insightful reports and helpful comments, and the editor for handling our manuscript. We have addressed all comments in this revision and provide our responses below. All changes in the manuscript are highlighted in \af{red} color.

\bigskip

\noindent

\begin{itemize}

\item consider methods to approximate the matrix functions without the need to use a quadrature formula (which can be easily done, here) and compare these methods to
the ones proposed so far.
\af{We have included a comparison with the standard Arnoldi approximation (equation (3.6)) in the experiments, and have clarified this in the experiments section (it may not have been clear in the first draft). Note we cannot compare our results to methods which use deflated restarting since the methods here cannot be restarted, and one cycle of a deflated restarted method is equivalent to the standard Arnoldi approximation. Furthermore, deflated restarted methods cannot be used to solve a sequence of problems with changing matrices and right hand sides.}

\item page 2, line 41: ’augmentation’ instead of ’augmentaion’. \af{corrected}

\item page 6, line 207: ’on the most general form’ sounds better to me than ’off the most general form’. \af{corrected}

\item page 6: The general idea as proposed on page 6 might also include cases where the system (5.1) does not have
an unique solution. For example, $\mathcal{U} \cap \mathcal{V}_{j}$ might not be trivial or the spaces spanned by $V_{j}$ and $U$ are of an
unfortunate choice. The system might also be severely ill-conditioned. Some hints should be given to the reader
that this might happen and how this might be taken care of in an algorithm.
\af{We have added an additional paragraph to discuss this in the text.}

\item page 7, lines 239,230: The authors state in these lines that the proof of the equivalence of the statements in the
framed boxes were a trivial extension of the proof shown in [35] to the shifted case and were thus not repeated
here. This confused me quite a bit.
\af{The proof of this equivalence is indeed trivial, so we have removed the reference to the proof.}

\item page 9, line 292, ”...where C = AU ...”. This line refers to equation (6.2). But in equation (6.2), C and U do not
appear. The efficient computation of (6.2) is only mentioned in lines 298-300.

\af{Although $C$ and $U$ do not appear explicitly in equation (6.2), the projector $P_{\sigma}$ does, which in turn depends on $C$ and $U$. So in order to define $P_{\sigma}$ (as we do after the equation) we need to first define $C$.}

\item page 14, Proposition 8.1. It might be clearer to mention in the proposition that the basis U is assumed to be
orthogonal. This has not been a requirement in several discussions of the draft so far.
\af{done}

\item page 15, in experiment one. For the approximation with respect to the standard Arnoldi approximation (FOM),
does the approximation correspond to (m = 50) steps? Or did you use more steps here?
\af{yes, the Arnoldi approximation uses only $m$ basis vectors, whereas the recycling methods uses $m + k$. We have clarified this in the text.}

\item page 15, in experiment one. A stable method that would not use any quadrature (all three proposed methods
use quadrature) would probably be directly on the error level where the rFOM v1-3 algorithms end up.
\af{see next comment}

\item page 17, Figure 2. There are probably measures to improve the numerical stability of the methods rFOM 1 and
rFOM 3.

\af{Yes there is. Since we submitted this work there has been further improvements to the work of this paper in [40]. In particular, we developed a stable version of the algorithm that does not rely on quadrature, and can also exploit randomized sketching. We have added a paragraph to the conclusions to briefly discuss this. We still believe the work in this manuscript is an important stepping stone to the improved algorithms of [40], and still has merit for publication.}

\end{itemize}
